AQuaMoHo: Localized Low-Cost Outdoor Air Quality Sensing over a Thermo-Hygrometer

Efficient air quality sensing serves as one of the essential services provided in any recent smart city. Mostly facilitated by sparsely deployed Air Quality Monitoring Stations (AQMSs) that are difficult to install and maintain, the overall spatial variation heavily impacts air quality monitoring for locations far enough from these pre-deployed public infrastructures. To mitigate this, we in this paper propose a framework named AQuaMoHo that can annotate data obtained from a low-cost thermo-hygrometer (as the sole physical sensing device) with the AQI labels, with the help of additional publicly crawled Spatio-temporal information of that locality. At its core, AQuaMoHo exploits the temporal patterns from a set of readily available spatial features using an LSTM-based model and further enhances the overall quality of the annotation using temporal attention. From a thorough study of two different cities, we observe that AQuaMoHo can significantly help annotate the air quality data on a personal scale.

==> Section/RelatedWorkNew.tex <==
%%Editting PP
 




\section{Related work}
\label{Survey} \textcolor{blue}{ 
The critical condition of air has led to a wide array of research in understanding the air quality at cost-effective methods, especially in a data-driven manner \cite{zheng2013u}. The primary focus so far has been to extend the air pollution measurement across space \cite{HOEK20087561} or through time \cite{zheng2015forecasting}. In this section, we have comprehensively compiled the research on cost-effective systems and discussed state of the art for calibration challenges. Consequently, we emphasize the different spatial and temporal features used to understand the Spatio-temporal dynamics and availability in Low Middle-Income Countries (LMICs)}


\textcolor{blue}{The focal point to address is the variability of pollution \cite{tan2014characterizing, gu2018intracity}  due to urban geographic factors responsible, variation in traffic patterns \cite{matte2013monitoring}. Precise sensing instruments, unfortunately, fail to cover the area as there are not enough sensors. In India, according to CPCB's estimate, currently has only 4-8\% coverage\footnote{https://urbanemissions.info/}. As an alternative, the advent of low-cost sensing (LCS) has increased spatial and temporal coverage. LCS can be static as well as moveable. The mobility of these sensors introduces the concept of using movement patterns to increase coverage. These sensors are often used in tandem with other available measurements to quantify measurements in locations where they are not places. These measurements can be local statistics like traffic count \cite{matte2013monitoring}, pedestrian count \cite{catlett2017array}, population density \cite{zheng2013u}, land use/land cover \cite{shukla2020mapping}, number of pollution sources or meteorological features \cite{liu2020exploring} like temperature humidity,wind speed and wind direction. This, combined with time-based patterns, can help understand the spatial dynamics of air quality. A significant point to note LCS does these types of measurements at the cost of accuracy and consistency. LCS extend beyond just sensors, and inherently when we consider the system, the cost rises significantly \cite{peltier2021update}. The LCS network additionally consists of maintaining the network, the energy management, data collection challenges. Sensors with mobility introduce a different type of challenge as the measurement depends on the air's sampling rate. Local context, as a result, is essential to account for the changes in air movement owing to mobility which includes the local speed and the wind direction. There has been significant work done in calibration as the variability across sensors is non-linear and often hard to detect. Mobility introduces new parameters to look at to calibrate the device outputs. 
Developing a cost-effective low-cost sensor architecture that is scalable, reliable, robust is a challenge by itself.  
}
\subsection{Cost Effective Air Quality Sensing/Ubiquitous Sensing}{
Cost-effective air quality sensing encompasses various techniques through which we can estimate the air quality either by the raw value of pollutants or through the standardized Air Quality Index values. There have been extensive works in the development of portable yet robust air quality monitoring devices that can augment the existing AQMS~\cite{liu2020low,gulia2020sensor, purpleair-inc-2021}. Liu \textit{et. al.} \cite{liu2020low}, use sensors for measuring the $PM_{2.5}$ and carbon monoxide (CO) considering the calibration of only the CO sensor, 
affecting the device's reliability. Mobile sensing through drones, named  \textit{ Sensor-based Wireless Air Quality Monitoring Network} (SWAQMN), has been proposed by Gulia \textit{et. al.} \cite{gulia2020sensor} to monitor real-time concentration of $PM_x$s. Commercial devices such as 'Purple Air' \cite{purpleair-inc-2021} enables sensing of $PM_{2.5}$ which uses pre-calibrated laser sensors. \textcolor{blue}{Extensive research has been done in creating networks at a city-scale which consists of hundreds of sensors \cite{catlett2017array} to even thousands of sensors \cite{chen2017open}. \cite{catlett2017array} created such a network of multimodal sensing to capture the  Maintaining the consistency and stability of such networks is a costly affair despite the low cost of the sensor. \cite{peltier2021update} show that maintaining the consistency and accuracy of these sensors is not low cost in the long run. Nevertheless, the report agrees that it is a useful way for measuring the particulate concentrations in moderate environments, and there is ample scope for refinement of models at a much granular level, especially for downstream tasks like the assessment of human exposure and dataset generation for the analysis of long-term trends once the device has been calibrated.}

}

%Local Sensitivity, Area of Coverage,  deployment info, Number of Units deployed/Area, dimension, calibration issue, remarks, separate para for cost benefit analysis, avoid cost in the table,


\begin{table}[!htbp]
\caption{Survey of Systems}
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{|l|l|c|l|l|}
\hline
\textbf{Paper}                               
& \textbf{Type of Measurement}   
& \textbf{Primary} 
& \textbf{Physical Sensors} 
& \textbf{City, No of Sensors}  \\ \hline
U-Air \cite{zheng2013u}                                        
& PM2.5                          
& \cmark                
& BAM Samplers                  
& Beijing, 18     \\ \hline
Purple Air\footnote{https://www2.purpleair.com/}                                   
& PM2.5                          
& \cmark                
&  Plantower PMS5003                      
&      \\ \hline
Array of Things\cite{catlett2017array}                              
&  N$O_2$, $O_3$, Temp, Humidity 
& \cmark                
& AlphaSense                      
& Chicago, 105     \\ \hline
Lj Chen\cite{chen2017open}                                      
& PM2.5                 
& \cmark                
& PlanTower                      
& Taiwan, 1000+     \\ \hline
Koala Sensing \cite{liu2020low}                                
& PM2.5, CO                          
& \cmark                
& Plantower PMS1003                      
&      \\ \hline
Image Based Participatory Sensing\cite{liu2018third}            
& PM2.5                          
& \xmark                
& N/A                            
& Beijing, N/A     \\ \hline
AirCalypse \cite{pramanik2018aircalypse, pramanik2020aircalypse} 
& PM2.5                          
& \xmark                
& N/A                            
& New Delhi, N/A    \\ \hline
\end{tabular}%
}
\label{tab:my-table}
\end{table}



\iffalse
In this section, we present the works related to air quality monitoring and prediction from two different directions -- (a) development of devices for air quality monitoring, (b) AQI estimation.

\textbf{Development of Air Quality Monitoring Devices:}
Various works in the literature~\cite{liu2020low,gulia2020sensor, purpleair-inc-2021} aimed to develop portable and robust devices for air quality monitoring, which can augment the existing AQMSs. Liu \textit{et. al.} \cite{liu2020low}, use sensors for measuring the $PM_{2.5}$ and carbon monoxide (CO) considering the calibration of only the CO sensor, 
affecting the device's reliability. A drone-based \textit{Wireless Air Quality Monitoring Network} (SWAQMN) has been proposed by Gulia \textit{et. al.} \cite{gulia2020sensor} to monitor real-time concentration of $PM_x$s. Commercial devices such as 'Purple Air' \cite{purpleair-inc-2021} enables sensing of $PM_{2.5}$ which uses pre-calibrated laser sensors.
\fi



% Please add the following required packages to your document preamble:
% \usepackage{lscape}
\begin{table}[!htbp]
\caption{Related Work on Calibration}
\scriptsize
%\resizebox{.8\pdfpageheight}{!}{%
\centering
\begin{tabular}{|l|c|l|l|l|l|}
\hline
\textbf{Ref} &
  \textbf{Sensors} &
  \textbf{Reference Monitors} &
  \textbf{Model} &
  \textbf{Features} \\ \hline
{\cite{lee2019efficient}} &
  AirBox by Edimax & 
  \begin{tabular}[c]{@{}l@{}} Taiwan Environmental Protection \\ Administration (TWEPA) Stations\end{tabular}&
  \begin{tabular}[c]{@{}l@{}}Generalized Additive \\ Model (GAM)\end{tabular} &
  PM2.5, T, RH \\ \hline
{\cite{desouza2022calibrating}} &
  \begin{tabular}[c]{@{}l@{}}PM2.5 (“Love My Air” \\ network, Denver)\end{tabular} &
  FEM PM2.5 &
  \begin{tabular}[c]{@{}l@{}}21 ML algo each \\ with 4 correction \\ factors\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}PM2.5, T, RH, \\ Dew, Time variant \\ factors\end{tabular} \\ \hline
{\cite{wang2019calibration}} &
  \begin{tabular}[c]{@{}l@{}}Particle monitor \\ (HK-B3, Hike, China)\end{tabular} &
  MicroPEM monitor (RTI, America) &
  Random Forest &
  PM2.5, T, RH \\ \hline
{\cite{cavaliere2018development}} &
  AIRQuino &
  TSI DustTrak &
  Regression &
  PM2.5, PM10 \\ \hline
{\cite{zaidan2020intelligent}} &
  \begin{tabular}[c]{@{}l@{}}Clarity Corporation, \\ Berkeley, USA\end{tabular} &
  \begin{tabular}[c]{@{}l@{}} Monitor stations located at SMEAR\\ \& supersite Mäkelänkatu \end{tabular} &
  Regression &
  PM2.5 \\ \hline
{\cite{karaoghlanian2022low}} &
  PurpleAir PA-II-SD &
  Met One E-BAM PLUS &
  Regression &
  PM2.5, PM10 \\ \hline
{\cite{chu2020spatial}} &
  \begin{tabular}[c]{@{}l@{}} AirBox, with PMS5003\\ optical particulate matter \\ sensor\end{tabular} &
  TWEPA’s Air Monitoring Network &
  Spatial Regression &
  PM2.5 \\ \hline
{\cite{concas2021low}} &
  \begin{tabular}[c]{@{}l@{}}PMS5003, Sensirion \\ SPS30, and Honeywell\\ HPMA115S0\end{tabular} &
  BAM-1020 FEM monitor &
  Regression &
  PM2.5, RH \\ \hline
\end{tabular}
%}%
\label{tab:related_works_calibration}
\end{table}



\textbf{Calibration of the AQMD:}
\textcolor{blue}{
Air quality monitoring through low-cost sensor (LCS) have gained ample attention from researchers of different disciplines. Due to the sensitivity drift in LCS, the data reliability is uncertain. So, calibration of these air quality LCS has gained popularity in recent decades. %Calibration is the process of rectifying the error in the measurement of the sensors. 
Majorly there are two ways to calibrate the sensors, hard-calibration and soft-calibration.
A work by the authors in \cite{marathe2021currentsense} proposed \textit{CurrentSense}, a sensor fingerprint for detecting faults and drifts in environmental IoT sensors that could not be detected before without additional information. In their study, they used the concept that every electrical or electro-mechanical sensor draws current from the IoT device for its operation. By sampling the current drawn by the sensor, we can derive a unique electrical fingerprint that can distinguish between working, faulty, and malfunctioning sensors. The CurrentSense fingerprint can also be used to monitor sensor health and improve sensor data quality. It is non-intrusive and can be applied to a wide variety of sensors. Moreover, this approach mostly focuses on detection of the faults and drifts and after detection, the sensors are required to be brought to the lab for correction. In real practice the monitoring network can be very large and dynamic, calibrating and maintaining such a monitoring network is cumbersome. So, we generally opted for soft-calibration techniques and few of the recent works are as follows.
Authors in \cite{lee2019efficient} have proposed generalized additive (GAM) based model to calibrate the LCS by collecting the data from regulatory stations in Taiwan and LCS. They study their space and time bias to calibrate the LCS.} 
\textcolor{blue}{
The authors in \cite{desouza2022calibrating} use 21 learning algorithms and developed four correction factors for each. They also deployed their LCS with a gold-standard reference monitor to obtain the calibration equation. The developed equation is then deployed to the sensors of the network to obtain the temporal and spatial trends of the network.
Authors in \cite{wang2019calibration} use a MicroPEM monitor (RTI, America) as a standard measurement device for particulate matters to calibrate the Hike monitors. Machine learning technique followed by ten fold validation is used to obtain the concentration of particles. A similar work is performed by the authors in \cite{cavaliere2018development}, they deployed LCS in Florence near an official fixed air quality monitoring station and calibrated the LCS. 
}
\textcolor{blue}{
The authors in \cite{zaidan2020intelligent} have calibrated the meteorological parameters using linear dynamic model and the particulate matters are calibrated using non-linear models. Authors in \cite{karaoghlanian2022low} calibrate the PurpleAir PA-II-SD which can measure the concentration of $PM_{2.5}$, and $PM_{10}$. They have used two high fidelity Met One E-BAM PLUS placed at a single location in Beirut, Lebanon. The authors focus on  inter-sensor variability of PurpleAir sensors with their accuracy. They use two linear regression models, first model uses the entire dataset of the concentration and the second model uses the 90\% quantile range to the concentration for better result without outliers. Spatial varying parameters are considered by the authors in \cite{chu2020spatial} by using the LCS as well as regulatory stations. They performed regression analysis for explaining the variability of the biases from the LCS. A summary of the sensors used, reference stations, and techniques with feature list by the mentioned works is depicted in Table \ref{tab:related_works_calibration}. Apart from the above mentioned works a survey was conducted by \cite{concas2021low} which supplements the previous surveys and focuses on the operations required to implement the calibration pipeline and to analyse the effect of different sensing technologies on this pipeline. The aforementioned works deal with machine learning based calibration but, the hard calibration, sensitivity analysis, are also important for improving the sensing reliability when deployed in any outdoor environment. 
}



\iffalse
{Air quality monitoring through Low-Cost Sensor (LCS) have gained ample attention from researchers of different disciplines. Due to the sensitivity drift in LCS, the data reliability is promising. So, calibration of these air quality LCS has gained popularity in recent decades. %Calibration is the process of rectifying the error in the measurement of the sensors. 
Authors in \cite{lee2019efficient} have proposed generalized additive (GAM) based model to calibrate the LCS by collecting the data from regulatory stations in Taiwan and LCS. They study their space and time bias to calibrate the LCS.} %This technique is highly affected by the ambient temperature and humidity which has not been considered by the authors.

\textcolor{blue}{
The authors in \cite{desouza2022calibrating} develop four correction factors using 21 learning algorithms. They also deployed their LCS with a gold-standard reference monitor to obtain the calibration equation. The developed equation is then deployed to the sensors of the network to obtain the temporal and spatial trends of the network. For each 21 machine learning 4 correcting factors have been developed.
Authors in \cite{wang2019calibration} use a MicroPEM monitor (RTI, America) as a standard measurement device for particulate matters to calibrate the Hike monitors. Machine learning technique followed by tenfold validation is used to obtain the concentration of particles. A similar work is performed by the authors in \cite{cavaliere2018development}, they deployed LCS in Florence near an official fixed air quality monitoring station and calibrated the LCS.} 

\textcolor{blue}{The authors in \cite{zaidan2020intelligent} have calibrated the meteorological parameters using linear dynamic model and the particulate matters are calibrated using non-linear models. An LCS PurpleAir PA-II-SD which can measure the concentration of $PM_{2.5}$, and $PM_{10}$, is calibrated by the authors in \cite{karaoghlanian2022low}. They have used two high fidelity Met One E-BAM PLUS placed at a single location in Beirut, Lebanon. The authors focus on  inter-sensor
variability of PurpleAir sensors with their accuracy. They use two linear regression models, first model uses the entire dataset of the concentration and the second model uses the 90\% quantile range to the concentration for better result without outliers. Spatial varying parameters are considered by the authors in \cite{chu2020spatial} by using the LCS as well as regulatory stations. They performed regression analysis for explaining the variability of the biases from the LCS. Apart from the above mentioned works a survey was conducted by \cite{concas2021low} which supplements the previous surveys and focuses on the operations required to implement the calibration pipeline andto analyse the effect of different sensing technologies on this pipeline. The abovementioned works deal with machine learning based calibration but, the hard calibration, sensitivity analysis, are also important when deployed in any outdoor environment for improving the sensing reliability.}
\fi
\begin{table*}
\scriptsize
\centering
\caption{Comparison of the above mentioned state of the art work and \ourmethod{}}
\label{tab_survey}
\resizebox{\columnwidth}{!}{
{\begin{tabular}{|l|l|l|c|c|c|l|c|} 
\hline
\multicolumn{1}{|c|}{\multirow{2}{*}{\textbf{Reference}}} & \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{Objective}}} & \multicolumn{4}{c|}{\textbf{Input Feature Sources for Model Training}}   & \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{ML Model}}} & \multirow{2}{*}{\textbf{\#AQI class}}  \\ 
\cline{3-6}
\multicolumn{1}{|c|}{}                                    & \multicolumn{1}{c|}{}                                    & \multicolumn{1}{c|}{\textbf{Meteorological}} & \textbf{Demographic}                & \textbf{Traffic Flow}             & \textbf{PM2.5/10}                       & \multicolumn{1}{c|}{}                                          &                                        \\ 
\hline
Zheng et. al.~\cite{zheng2013u}                            & AQI estimation                                           & Public Website                               & \multicolumn{1}{l|}{POI, road~data} & \multicolumn{1}{l|}{3000 Taxis}   & \xmark                                    & CRF  ANN         & 4                  \\ 
\hline
Lin Yijun et. al.~\cite{lin2018exploiting}                        & PM2.5 forecasting                                        & Dark Sky API                                 & \multicolumn{1}{l|}{OSM}            & \xmark                              & \multicolumn{1}{l|}{Public AQMS}        & CONV-RNN                                                                          & \xmark                                   \\ 
\hline
Xu x et. al.~\cite{xu2019multitask}                             & PM2.5 estimation                                         & Meteorological stations                      & \xmark                                & \xmark                              & \multicolumn{1}{l|}{Public AQMS}        & LSTM-Autoencoder                                    & \xmark                                   \\ 
\hline
Gu Ke et. al.~\cite{gu2018recurrent}                            & Air quality forecasting                                  & Self-deployed AQMSs                          & \xmark                                & \xmark                              & \multicolumn{1}{l|}{Self-deployed AQMS} & RAQP                 & \xmark                                   \\ 
\hline
Kaya et. al.~\cite{kaya2020deep}                             & PM10 forecasting                                         & Meteorological stations                      & \xmark                                & \multicolumn{1}{l|}{Traffic data} & \multicolumn{1}{l|}{Public AQMS}        & DFS         & \xmark                                   \\ 
\hline
Kleine et. al.~\cite{kleine2017modeling}                           & AQI estimation                                           & Meteorological stations                      & \xmark                                & \xmark                              & \xmark                                    & BT, L-SVM    & 3                                      \\ 
\hline
\ourmethod{} (Our)                                                 & AQI annotation                                           & THM, OpenWeather API                         & \multicolumn{1}{l|}{Gmaps API}      & \xmark                              & \xmark                                    & Random Forest  & 5                                      \\
\hline

\end{tabular}}
}
\end{table*}




\textbf{AQI Estimation:} 
Several works have used machine learning-based Spatio-temporal modelling to predict air pollution across a city. Zheng \textit{et. al.}~\cite{zheng2013u} have used a co-training approach to combine a spatial and a temporal classifier to estimate the AQI from various auxiliary data. In~\cite{lin2018exploiting}, the authors have proposed a diffusion convolution RNN model to forecast $PM_{2.5}$ particles for the next $24$ hours at a given location, based on the meteorological and geographic data. In~\cite{xu2019multitask}, the authors have used a multi-layer LSTM and a stacked auto-encoder to estimate the pollution level from meteorological data, 
considering only local information, hence fails to capture the spatial spread of pollutants. Several works in the literature~\cite{kleine2017modeling,al2017prediction,qi2018deep,gu2018recurrent} have established the correlation among various meteorological data, like temperature, pressure, wind speed, wind direction, among others, and proposed machine learning classifiers to predict the AQI. Other existing works~\cite{wu2019msstn,yi2018deep,han2018umeair,zheng2015forecasting,kok2017deep} require a high volume of ground truth data and are particularly focused on temporal forecasting of pollutants rather than understanding the spatial distribution of the AQI over demography. Kaya \textit{et. al.}~\cite{kaya2020deep} have used meteorological, pollutant, and traffic data to forecast the concentration of $PM_{10}$ using a flexible deep model. The majority of these works demand continuous sensing of auxiliary information and assume uniformly available AQMS data across different city regions, which may not be available in most global cities. 

 Our system \ourmethod{} addressed the limitations of the existing works and provided an integrated framework ensuring the design of reliable sensing devices and developing suitable models for a city-wide fine-grained AQI annotation, providing an accuracy of more than 60\%. \ourmethod{}, apart from the GPS coordinates of the target location, requires minimal input from the user viz., temperature, humidity using a relatively low-cost device such as a simple THM (\textasciitilde 40 USD) compared to a direct sensing device like Purple Air (> 240 USD). A summary of the state of the art methods is mentioned in Table \ref{tab_survey} and compared with \ourmethod{} based on their objective, features source, ML model, and the number of AQI classes.

==> Section/oldRelatedWork.tex <==
\begin{table*}
\scriptsize
\centering
\caption{Comparison of the above mentioned state of the art work and \ourmethod{}}
\label{tab_survey}
{\begin{tabular}{|l|l|l|c|c|c|l|c|} 
\hline
\multicolumn{1}{|c|}{\multirow{2}{*}{\textbf{Reference}}} & \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{Objective}}} & \multicolumn{4}{c|}{\textbf{Input Feature Sources for Model Training}}   & \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{ML Model}}} & \multirow{2}{*}{\textbf{\#AQI class}}  \\ 
\cline{3-6}
\multicolumn{1}{|c|}{}                                    & \multicolumn{1}{c|}{}                                    & \multicolumn{1}{c|}{\textbf{Meteorological}} & \textbf{Demographic}                & \textbf{Traffic Flow}             & \textbf{PM2.5/10}                       & \multicolumn{1}{c|}{}                                          &                                        \\ 
\hline
Zheng et. al.~\cite{zheng2013u}                            & AQI estimation                                           & Public Website                               & \multicolumn{1}{l|}{POI, road~data} & \multicolumn{1}{l|}{3000 Taxis}   & \xmark                                    & CRF  ANN         & 4                  \\ 
\hline
Lin Yijun et. al.~\cite{lin2018exploiting}                        & PM2.5 forecasting                                        & Dark Sky API                                 & \multicolumn{1}{l|}{OSM}            & \xmark                              & \multicolumn{1}{l|}{Public AQMS}        & CONV-RNN                                                                          & \xmark                                   \\ 
\hline
Xu x et. al.~\cite{xu2019multitask}                             & PM2.5 estimation                                         & Meteorological stations                      & \xmark                                & \xmark                              & \multicolumn{1}{l|}{Public AQMS}        & LSTM-Autoencoder                                    & \xmark                                   \\ 
\hline
Gu Ke et. al.~\cite{gu2018recurrent}                            & Air quality forecasting                                  & Self-deployed AQMSs                          & \xmark                                & \xmark                              & \multicolumn{1}{l|}{Self-deployed AQMS} & RAQP                 & \xmark                                   \\ 
\hline
Kaya et. al.~\cite{kaya2020deep}                             & PM10 forecasting                                         & Meteorological stations                      & \xmark                                & \multicolumn{1}{l|}{Traffic data} & \multicolumn{1}{l|}{Public AQMS}        & DFS         & \xmark                                   \\ 
\hline
Kleine et. al.~\cite{kleine2017modeling}                           & AQI estimation                                           & Meteorological stations                      & \xmark                                & \xmark                              & \xmark                                    & BT, L-SVM    & 3                                      \\ 
\hline
\ourmethod{} (Our)                                                 & AQI annotation                                           & THM, OpenWeather API                         & \multicolumn{1}{l|}{Gmaps API}      & \xmark                              & \xmark                                    & Random Forest  & 5                                      \\
\hline
\end{tabular}}
\end{table*}
\section{Related work}
\label{Survey}

In this section, we present the works related to air quality monitoring and prediction from two different directions -- (a) development of devices for air quality monitoring, (b) AQI estimation.

\textbf{Development of Air Quality Monitoring Devices:}
Various works in the literature~\cite{liu2020low,gulia2020sensor, }%purpleair-inc-2021} 
aimed to develop portable and robust devices for air quality monitoring, which can augment the existing AQMSs. Liu \textit{et. al.} \cite{liu2020low}, use sensors for measuring the $PM_{2.5}$ and carbon monoxide (CO) considering the calibration of only the CO sensor, thereby 
affecting the device's reliability. A drone-based \textit{Wireless Air Quality Monitoring Network} (SWAQMN) has been proposed by Gulia \textit{et. al.} \cite{gulia2020sensor} to monitor real-time concentration of $PM_x$s. Commercial devices such as 'Purple Air' %\cite{purpleair-inc-2021} 
enables sensing of $PM_{2.5}$ which uses pre-calibrated laser sensors.

\textbf{AQI Estimation:} 
Several works have used machine learning-based spatio-temporal modeling to predict air pollution across a city. Zheng \textit{et. al.}~\cite{zheng2013u} have used a co-training approach to combine a spatial and a temporal classifier to estimate the AQI from various auxiliary data.  In~\cite{lin2018exploiting}, the authors have proposed a diffusion convolution RNN model to forecast $PM_{2.5}$ particles for the next $24$ hours at a given location, based on the meteorological and geographic data. In~\cite{xu2019multitask}, the authors have used a multi-layer LSTM and a stacked auto-encoder to estimate the pollution level from meteorological data, 
considering only local information, hence fails to capture the spatial spread of pollutants. Several works in the literature~\cite{kleine2017modeling,al2017prediction,qi2018deep,gu2018recurrent} have established the correlation among various meteorological data, like temperature, pressure, wind speed, wind direction, etc., and proposed machine learning classifiers to predict the AQI. Other existing works~\cite{wu2019msstn,yi2018deep,han2018umeair,zheng2015forecasting,kok2017deep} require a high volume of ground truth data, and are particularly focused on temporal forecasting of pollutants rather than understanding the spatial distribution of the AQI over demography. Kaya \textit{et. al.}~\cite{kaya2020deep} have used meteorological, pollutant, and traffic data to forecast the concentration of $PM_{10}$ using flexible deep model. The majority of these works demand continuous sensing of auxiliary information and assume uniformly available AQMS data across different city regions, which may not be available in most cities across the globe. 

 Our system \ourmethod{} addressed the limitations of the existing works and provided an integrated framework ensuring the design of reliable sensing devices, and developing suitable models for a city-wide fine-grained AQI annotation, providing an accuracy more than 60\%. \ourmethod{}, apart from the GPS coordinates of the target location, requires minimal input from the user viz., temperature, humidity using relatively low-cost device such as a simple THM (\textasciitilde 40 USD) compared to a direct sensing device like Purple Air (> 240 USD). A summary of the state of the art methods are mentioned in the Table \ref{tab_survey} and compared with \ourmethod{} based on their objective, features source, ML model, and the number of AQI classes.

==> Section/oldRelatedWorkNew__.tex <==
%%Editting PP
 




\section{Related work}
\label{Survey} \textcolor{red}{ 
The critical condition of air has led to a wide array of research in understanding the air quality at cost effective methods especially in a data driven manner \cite{zheng2013u}. The primary focus so far has been to extend the air pollution measurement across space \cite{HOEK20087561} or through time \cite{zheng2015forecasting}. In this section, we have comprehensively compiled the research on cost-effective systems and discuss on the state of the art for the calibration challenges. Consequently, we emphasise upon the different the spatial and temporal features used to understand the spatio-temporal dynamics and availability in Low Middle Income Countries (LMICs)}


\textcolor{red}{The focal point to address is the variability of pollution \cite{tan2014characterizing, gu2018intracity}  due to urban geographic factors responsible, variation in traffic patterns \cite{matte2013monitoring}. Precise sensing instruments unfortunately fail to cover the area as there are not enough sensors. In India, according to CPCB's own estimate currently has only 4-8\% coverage\footnote{https://urbanemissions.info/}. As an alternative the advent of low cost sensing (LCS), has increased the spatial and temporal coverage. LCS can be static as well as moveable. Mobility of these sensors introduces the concept of using movement patterns to increase coverage. These sensors are often used in tandem with other available measurement to quantify measurements in locations where they are not places. These measurements can be local statistics like traffic count \cite{matte2013monitoring}, pedestrian count \cite{catlett2017array}, population density \cite{zheng2013u}, land use/land cover \cite{shukla2020mapping}, number of pollution sources or meteorological features \cite{liu2020exploring} like temperature humidity,wind speed and wind direction. This combined with time based patterns can help in understanding the spatial dynamics of air quality. A significant point to note LCS does these types of measurement at the cost of accuracy and consistency. LCS extend beyond just sensors and inherently when we consider the system, the cost rises significantly \cite{peltier2021update}.  The LCS network additionally consists of maintaining the network, the energy management, data collection challenges. Sensors with mobility introduces a different type of challenge as the measurement is dependent on the sampling rate of the air. Local context as a result is very important to account for the changes in air movement owing to mobility which includes the local speed and the wind direction. To that end, there has been significant work done in calibration as the variability across sensors are non-linear and is often hard to detect. Mobility introduces new parameters to look at to calibrate the device outputs. 
The development of a cost-effective low-cost sensor architecture which is scaleable, reliable, robust is a challenge by itself.  
}
\subsection{Cost Effective Air Quality Sensing/Ubiquitous Sensing}{
Cost effective air quality sensing encompasses various techniques through which we can estimate the air quality either by the raw value of pollutants or through the standardized Air Quality Index values. There have been extensive works in development of portable yet robust air quality monitoring devices which can augment the existing AQMS~\cite{liu2020low,gulia2020sensor, purpleair-inc-2021}. Liu \textit{et. al.} \cite{liu2020low}, use sensors for measuring the $PM_{2.5}$ and carbon monoxide (CO) considering the calibration of only the CO sensor, 
affecting the device's reliability. Mobile sensing through drones, named  \textit{ Sensor-based Wireless Air Quality Monitoring Network} (SWAQMN) has been proposed by Gulia \textit{et. al.} \cite{gulia2020sensor} to monitor real-time concentration of $PM_x$s. Commercial devices such as 'Purple Air' \cite{purpleair-inc-2021} enables sensing of $PM_{2.5}$ which uses pre-calibrated laser sensors. \textcolor{red}{Extensive research have been done in creating networks at city scale which consists of hundreds of sensors \cite{catlett2017array} to even thousands of sensors \cite{chen2017open}. Maintaining the consistency and stability of such networks is a costly affair despite the low cost of the sensor. \cite{peltier2021update} show that maintaining the consistency and accuracy of these sensors is not low cost in the long run. But the report agrees that it is a useful way for measuring the particulate concentrations in moderate environments and there is ample scope for refinement of models at a much granular level especially for downstream tasks like the assessment of human exposure and data-set generation for the analysis of long-term trends once the device has been calibrated.}

}

% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{|l|l|l|l|l|l|}
\hline
\textbf{Paper}                               & \textbf{Type of Measurement}   & \textbf{Primary} & \textbf{Physical Sensors Used} & \textbf{Scale {[}{]}} & Cost \\ \hline
U-Air \cite{zheng2013u}                                        & PM2.5                          & Y                & BAM Samplers                   &                       &      \\ \hline
Purple Air\footnote{https://www2.purpleair.com/}                                   & PM2.5                          & Y                & PlanTower                      &                       &      \\ \hline
Array of Things\cite{catlett2017array}                              & PM2.5, NO2, O3, Temp, Humidity & Y                & PlanTower                      &                       &      \\ \hline
Lj Chen\cite{chen2017open}                                      & PM2.5                          & Y                & PlanTower                      &                       &      \\ \hline
Koala Sensing \cite{liu2020low}                                & PM2.5                          & Y                & PlanTower                      &                       &      \\ \hline
Image Based Participatory Sensing\cite{liu2018third}            & PM2.5                          & N                & N/A                            &                       &      \\ \hline
AirCalypse \cite{pramanik2018aircalypse, pramanik2020aircalypse} & PM2.5                          & N                & N/A                            &                       &      \\ \hline
                                            %  &                                &                  &                                &                       &      \\ \hline
                                            %  &                                &                  &                                &                       &      \\ \hline
\end{tabular}%
}
\caption{Survey of Systems}
\label{tab:my-table}
\end{table}


\begin{table}[!htbp]
\centering
\resizebox{.65\textwidth}{!}{%
\begin{tabular}{|l|l|l|l|}
\hline
\textbf{Feature} & \textbf{Spatial} & \textbf{Temporal} & \textbf{Availability in LMIC} \\ \hline
Road Network \cite{matte2013monitoring} & Y & N & N  \\ \hline
Traffic Count \cite{catlett2017array} & Y & Y & N   \\ \hline
Meteorology: Temperature & Y & Y & Y  \\ \hline
Meteorology: Humidity & Y & Y & Y  \\ \hline
Feels Like & Y & Y & Y  \\ \hline
Temperature\_Min & Y & Y & Y  \\ \hline
Temperature Max & Y & Y & Y  \\ \hline
Wind Speed & Y & Y & Y   \\ \hline
Wind Direction & Y & Y & Y   \\ \hline
Rain/Precipitation & Y & Y & Y   \\ \hline
Cloud & Y & Y & Y   \\ \hline
Day of the Week & N & Y & Y   \\ \hline
Time of the day & N & Y & Y   \\ \hline
Year & N & Y & Y   \\ \hline
Month & N & Y & Y   \\ \hline
Land Use/ Land Cover & Y & N & N   \\ \hline
\end{tabular}
}%
\caption{List of Features}
\label{tab:related_works_calibration}
\end{table}




\iffalse
In this section, we present the works related to air quality monitoring and prediction from two different directions -- (a) development of devices for air quality monitoring, (b) AQI estimation.

\textbf{Development of Air Quality Monitoring Devices:}
Various works in the literature~\cite{liu2020low,gulia2020sensor, purpleair-inc-2021} aimed to develop portable and robust devices for air quality monitoring, which can augment the existing AQMSs. Liu \textit{et. al.} \cite{liu2020low}, use sensors for measuring the $PM_{2.5}$ and carbon monoxide (CO) considering the calibration of only the CO sensor, 
affecting the device's reliability. A drone-based \textit{Wireless Air Quality Monitoring Network} (SWAQMN) has been proposed by Gulia \textit{et. al.} \cite{gulia2020sensor} to monitor real-time concentration of $PM_x$s. Commercial devices such as 'Purple Air' \cite{purpleair-inc-2021} enables sensing of $PM_{2.5}$ which uses pre-calibrated laser sensors.
\fi



% Please add the following required packages to your document preamble:
% \usepackage{lscape}
\begin{landscape}
\begin{table}[]
\resizebox{.8\pdfpageheight}{!}{%
\centering
\begin{tabular}{|l|l|l|l|l|l|l|l|}
\hline
\textbf{Ref} &
  \textbf{Developed LCS?} &
  \textbf{Sensors Used} &
  \textbf{Regulatory Station} &
  \textbf{Model Used} &
  Features Used &
  \begin{tabular}[c]{@{}l@{}}Hard \\ calibration\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}Indoor/Outdoor \\ Environment\end{tabular} \\ \hline
{\cite{lee2019efficient}} &
  Y &
  PM2.5 &
  Y (Taiwan) &
  \begin{tabular}[c]{@{}l@{}}Generalized Additive \\ Model (GAM)\end{tabular} &
  Ref PM2.5 &
  N &
  Outdoor \\ \hline
{\cite{desouza2022calibrating}} &
  N &
  \begin{tabular}[c]{@{}l@{}}PM2.5 (“Love My Air” \\ network, Denver)\end{tabular} &
  Y (FEM PM2.5) &
  \begin{tabular}[c]{@{}l@{}}22 ML algo each \\ with 4 correction \\ factors\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}PM2.5, T, RH, \\ Dew, Time variant \\ factors\end{tabular} &
  N &
  Outdoor \\ \hline
{\cite{wang2019calibration}} &
  N &
  \begin{tabular}[c]{@{}l@{}}Particle monitor \\ (HK-B3, Hike, China)\end{tabular} &
  MicroPEM monitor (RTI, America) &
  Random forest &
  PM2.5, T, RH &
  N &
  Outdoor \\ \hline
{\cite{cavaliere2018development}} &
  N &
  AIRQuino &
  TSI DustTrak &
  Regression &
  PM2.5, PM10 &
  N &
  Outdoor \\ \hline
{\cite{zaidan2020intelligent}} &
  Y &
  \begin{tabular}[c]{@{}l@{}}Clarity Corporation, \\ Berkeley, USA\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}Station for Measuring Ecosystem-\\ Atmosphere Relations, Supersite \\ monitoring station (we denote as \\ M), operated by Helsinki Region \\ Environmental Services\\ Authority\end{tabular} &
  Regression &
  PM2.5, &
  N &
  Outdoor \\ \hline
{\cite{karaoghlanian2022low}} &
  N &
  PurpleAir PA-II-SD &
  Met One E-BAM PLUS &
  Regression &
  PM2.5, PM10 &
  N &
  Outdoor \\ \hline
{\cite{chu2020spatial}} &
  N &
  \begin{tabular}[c]{@{}l@{}}AirBox, with \\ PMS5003 optical \\ particulate matter \\ sensor\end{tabular} &
  TWEPA’s Air Monitoring Network &
  Spatial Regression &
  PM2.5, &
  N &
  Outdoor \\ \hline
{\cite{concas2021low}} &
  N &
  \begin{tabular}[c]{@{}l@{}}PMS5003, Sensirion \\ SPS30, and Honeywell\\ HPMA115S0\end{tabular} &
  BAM-1020 FEM monitor &
  Regression &
  PM2.5, RH &
  N &
  Outdoor \\ \hline
{\cite{marathe2021currentsense}} &
  N &
  \begin{tabular}[c]{@{}l@{}}Raw Sensors\\ (PM2.5, Temp, \\ CO2, VOC)\end{tabular} &
  NA &
  NA &
  NA &
  Y &
  \begin{tabular}[c]{@{}l@{}}Indoor/\\ Outdoor\end{tabular} \\ \hline
\end{tabular}
}%
\caption{Related Work on Calibration}
\label{tab:related_works_calibration}
\end{table}
\end{landscape}



\textbf{Calibration of the AQMD:}
\textcolor{red}{Air quality monitoring through low-Cost Sensor (LCS) have gained ample attention from researchers of different disciplines. Due to the sensitivity drift in LCS, the data reliability is promising. So, calibration of these air quality LCS has gained popularity in recent decades. //Calibration is the process of rectifying the error in the measurement of the sensors. 
Authors in [1] have proposed a generalized additive (GAM) based model to calibrate the LCS by collecting the data from regulatory stations in Taiwan and LCS. They study their space and time bias to calibrate the LCS. 
//This technique is highly affected by the ambient temperature and humidity which has not been considered by the authors.}

\textcolor{red}{DeSouza P. et al. [2] develop four correction factors using 21 learning algorithms. They also deployed their LCS with a gold-standard reference monitor to obtain the calibration equation. The developed equation is then deployed to the sensors of the network to obtain the temporal and spatial trends of the network. For each 21 machine learning 4 correcting factors have been developed.}
\textcolor{red}{Authors in [3] use a MicroPEM monitor (RTI, America) as a standard measurement device for particulate matters to calibrate the Hike monitors. Machine learning technique followed by ten fold validation is used to obtain the concentration of particles. A similar work is performed by the authors in [5] et al., they deployed LCS in Florence near an official fixed air quality monitoring station and calibrated the LCS.}

\textcolor{red}{The authors in [6] have calibrated the meteorological parameters using linear dynamic model and the particulate matters are calibrated using non-linear models.Most recently developed LCS PurpuleAir is calibrated in a work by [8], they have used two high fidelity Met One E-BAM PLUS placed at a single location in Beirut, Lebanon. The authors focus on  inter-sensor variability of PurpleAir sensors with their accuracy. They use two linear regression models, first model uses the entire dataset of the concentration and the second model uses the 90\% quantile range to the concentration for better results without outliers. Spatial varying parameters are considered by the authors in [9] by using the LCS as well as regulatory stations. They performed regression analysis for explaining the variability of the biases from the LCS. Apart from the above mentioned works a survey was conducted by [11] which supplements the previous surveys and focuses on the operations required to implement the calibration pipeline and to analyse the effect of different sensing technologies on this pipeline. The above mentioned works deal with machine learning based calibration but, the hard calibration, sensitivity analysis, are also important when deployed in any outdoor environment for improving the sensing reliability. }


\iffalse
{Air quality monitoring through low-Cost Sensor (LCS) have gained ample attention from researchers of different disciplines. Due to the sensitivity drift in LCS, the data reliability is promising. So, calibration of these air quality LCS has gained popularity in recent decades. %Calibration is the process of rectifying the error in the measurement of the sensors. 
Authors in \cite{lee2019efficient} have proposed generalized additive (GAM) based model to calibrate the LCS by collecting the data from regulatory stations in Taiwan and LCS. They study their space and time bias to calibrate the LCS.} %This technique is highly affected by the ambient temperature and humidity which has not been considered bu the authors.

\textcolor{red}{
The authors in \cite{desouza2022calibrating} develop four correction factors using 21 learning algorithms. They also deployed their LCS with a gold-standard reference monitor to obtain the calibration equation. The developed equation is then deployed to the sensors of the network to obtain the temporal and spatial trends of the network. For each 21 machine learning 4 correcting factors have been developed.
Authors in \cite{wang2019calibration} use a MicroPEM monitor (RTI, America) as a standard measurement device for particulate matters to calibrate the Hike monitors. Machine learning technique followed by ten fold validation is used to obtain the concentration of particles. A similar work is performed by the authors in \cite{cavaliere2018development}, they deployed LCS in Florence near an official fixed air quality monitoring station and calibrated the LCS.} 

\textcolor{red}{The authors in \cite{zaidan2020intelligent} have calibrated the meteorological parameters using linear dynamic model and the particulate matters are calibrated using non-linear models. An LCS PurpleAir PA-II-SD which can measure the concentration of $PM_{2.5}$, and $PM_{10}$, is calibrated by the authors in \cite{karaoghlanian2022low}. They have used two high fidelity Met One E-BAM PLUS placed at a single location in Beirut, Lebanon. The authors focus on  inter-sensor
variability of PurpleAir sensors with their accuracy. They use two linear regression models, first model uses the entire dataset of the concentration and the second model uses the 90\% quantile range to the concentration for better result without outliers. Spatial varying parameters are considered by the authors in \cite{chu2020spatial} by using the LCS as well as regulatory stations. They performed regression analysis for explaining the variability of the biases from the LCS. Apart from the above mentioned works a survey was conducted by \cite{concas2021low} which supplements the previous surveys and focuses on the operations required to implement the calibration pipeline andto analyse the effect of different sensing technologies on this pipeline. The abovementioned works deal with machine learning based calibration but, the hard calibration, sensitivity analysis, are also important when deployed in any outdoor environment for improving the sensing reliability.}
\fi
\begin{table*}
\scriptsize
\centering
\caption{Comparison of the above mentioned state of the art work and \ourmethod{}}
\label{tab_survey}
\resizebox{\columnwidth}{!}{
{\begin{tabular}{|l|l|l|c|c|c|l|c|} 
\hline
\multicolumn{1}{|c|}{\multirow{2}{*}{\textbf{Reference}}} & \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{Objective}}} & \multicolumn{4}{c|}{\textbf{Input Feature Sources for Model Training}}   & \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{ML Model}}} & \multirow{2}{*}{\textbf{\#AQI class}}  \\ 
\cline{3-6}
\multicolumn{1}{|c|}{}                                    & \multicolumn{1}{c|}{}                                    & \multicolumn{1}{c|}{\textbf{Meteorological}} & \textbf{Demographic}                & \textbf{Traffic Flow}             & \textbf{PM2.5/10}                       & \multicolumn{1}{c|}{}                                          &                                        \\ 
\hline
Zheng et. al.~\cite{zheng2013u}                            & AQI estimation                                           & Public Website                               & \multicolumn{1}{l|}{POI, road~data} & \multicolumn{1}{l|}{3000 Taxis}   & \xmark                                    & CRF  ANN         & 4                  \\ 
\hline
Lin Yijun et. al.~\cite{lin2018exploiting}                        & PM2.5 forecasting                                        & Dark Sky API                                 & \multicolumn{1}{l|}{OSM}            & \xmark                              & \multicolumn{1}{l|}{Public AQMS}        & CONV-RNN                                                                          & \xmark                                   \\ 
\hline
Xu x et. al.~\cite{xu2019multitask}                             & PM2.5 estimation                                         & Meteorological stations                      & \xmark                                & \xmark                              & \multicolumn{1}{l|}{Public AQMS}        & LSTM-Autoencoder                                    & \xmark                                   \\ 
\hline
Gu Ke et. al.~\cite{gu2018recurrent}                            & Air quality forecasting                                  & Self-deployed AQMSs                          & \xmark                                & \xmark                              & \multicolumn{1}{l|}{Self-deployed AQMS} & RAQP                 & \xmark                                   \\ 
\hline
Kaya et. al.~\cite{kaya2020deep}                             & PM10 forecasting                                         & Meteorological stations                      & \xmark                                & \multicolumn{1}{l|}{Traffic data} & \multicolumn{1}{l|}{Public AQMS}        & DFS         & \xmark                                   \\ 
\hline
Kleine et. al.~\cite{kleine2017modeling}                           & AQI estimation                                           & Meteorological stations                      & \xmark                                & \xmark                              & \xmark                                    & BT, L-SVM    & 3                                      \\ 
\hline
\ourmethod{} (Our)                                                 & AQI annotation                                           & THM, OpenWeather API                         & \multicolumn{1}{l|}{Gmaps API}      & \xmark                              & \xmark                                    & Random Forest  & 5                                      \\
\hline

\end{tabular}}
}
\end{table*}




\textbf{AQI Estimation:} 
Several works have used machine learning-based spatio-temporal modeling to predict air pollution across a city. Zheng \textit{et. al.}~\cite{zheng2013u} have used a co-training approach to combine a spatial and a temporal classifier to estimate the AQI from various auxiliary data.  In~\cite{lin2018exploiting}, the authors have proposed a diffusion convolution RNN model to forecast $PM_{2.5}$ particles for the next $24$ hours at a given location, based on the meteorological and geographic data. In~\cite{xu2019multitask}, the authors have used a multi-layer LSTM and a stacked auto-encoder to estimate the pollution level from meteorological data, 
considering only local information, hence fails to capture the spatial spread of pollutants. Several works in the literature~\cite{kleine2017modeling,al2017prediction,qi2018deep,gu2018recurrent} have established the correlation among various meteorological data, like temperature, pressure, wind speed, wind direction, etc., and proposed machine learning classifiers to predict the AQI. Other existing works~\cite{wu2019msstn,yi2018deep,han2018umeair,zheng2015forecasting,kok2017deep} require a high volume of ground truth data, and are particularly focused on temporal forecasting of pollutants rather than understanding the spatial distribution of the AQI over demography. Kaya \textit{et. al.}~\cite{kaya2020deep} have used meteorological, pollutant, and traffic data to forecast the concentration of $PM_{10}$ using flexible deep model. The majority of these works demand continuous sensing of auxiliary information and assume uniformly available AQMS data across different city regions, which may not be available in most cities across the globe. 

 Our system \ourmethod{} addressed the limitations of the existing works and provided an integrated framework ensuring the design of reliable sensing devices, and developing suitable models for a city-wide fine-grained AQI annotation, providing an accuracy more than 60\%. \ourmethod{}, apart from the GPS coordinates of the target location, requires minimal input from the user viz., temperature, humidity using relatively low-cost device such as a simple THM (\textasciitilde 40 USD) compared to a direct sensing device like Purple Air (> 240 USD). A summary of the state of the art methods are mentioned in the Table \ref{tab_survey} and compared with \ourmethod{} based on their objective, features source, ML model, and the number of AQI classes.
